On the Role of Discount Factor in Offline Reinforcement Learning

Offline reinforcement learning (RL) enables effective learning from previously collected data without exploration, which shows great promise in real-world applications when exploration is expensive or even infeasible. The discount factor, $\gamma$, plays a vital role in improving online RL sample efficiency and estimation accuracy, but the role of the discount factor in offline RL is not well explored. This paper examines two distinct effects of $\gamma$ in offline RL with theoretical analysis, namely the regularization effect and the pessimism effect. On the one hand, $\gamma$ is a regulator to trade-off optimality with sample efficiency upon existing offline techniques. On the other hand, lower guidance $\gamma$ can also be seen as a way of pessimism where we optimize the policy's performance in the worst possible models. We empirically verify the above theoretical observation with tabular MDPs and standard D4RL tasks. The results show that the discount factor plays an essential role in the performance of offline RL algorithms, both under small data regimes upon existing offline methods and in large data regimes without other conservative methods.

==> experiments.tex <==
\section{Empirical Results}
The goal of the experiments in this section is to investigate the following questions.
Can the adjusted guidance discount factor improve the performance of current offline RL algorithms?
Can the smaller guidance discount factor improve the performance of online RL algorithms on offline tasks? 
How is the optimal discount factor related to data size?
What is the benefit of changing the discount factor compared to the algorithm's original parameter?

\subsection{Toy example}
123

\subsection{Experimental results on D4RL tasks}
\subsubsection{Experimental results of offline algorithms}

\begin{figure*}[t]
    \centering
    \subfigure{
    \includegraphics[scale=0.125]{50+x-summary/walker2d.pdf}}
    \hspace{-3.5mm}
    \subfigure{
    \includegraphics[scale=0.125]{50+x-2/walker2d-medium-v2-50-0.pdf}}
    \hspace{-3.5mm}
    \subfigure{
    \includegraphics[scale=0.125]{50+x-2/walker2d-medium-v2-50-5.pdf}}
    \hspace{-3.5mm}
    \subfigure{
    \includegraphics[scale=0.125]{50+x-2/walker2d-medium-v2-50-10.pdf}}
    \hspace{-3.5mm}
    \subfigure{
    \includegraphics[scale=0.125]{50+x-2/walker2d-medium-v2-50-15.pdf}}
    \hspace{-3.5mm}
    %\subfigure{
    %\includegraphics[scale=0.125]{50+x-2/walker2d-medium-v2-50-20.pdf}}
    %\hspace{-3.5mm}
    \subfigure{
    \includegraphics[scale=0.125]{50+x-2/walker2d-medium-v2-50-25.pdf}}
    
    \subfigure{
    \includegraphics[scale=0.125]{50+x-summary/hopper.pdf}}
    \hspace{-3.5mm}
    \subfigure{
    \includegraphics[scale=0.125]{50+x-2/hopper-medium-v2-50-0.pdf}}
    \hspace{-3.5mm}
    \subfigure{
    \includegraphics[scale=0.125]{50+x-2/hopper-medium-v2-50-5.pdf}}
    \hspace{-3.5mm}
    \subfigure{
    \includegraphics[scale=0.125]{50+x-2/hopper-medium-v2-50-10.pdf}}
    \hspace{-3.5mm}
    \subfigure{
    \includegraphics[scale=0.125]{50+x-2/hopper-medium-v2-50-15.pdf}}
    \hspace{-3.5mm}
    %\subfigure{
    %\includegraphics[scale=0.125]{50+x-2/hopper-medium-v2-50-20.pdf}}
    %\hspace{-3.5mm}
    \subfigure{
    \includegraphics[scale=0.125]{50+x-2/hopper-medium-v2-50-25.pdf}}
    
    \subfigure{
    \includegraphics[scale=0.125]{50+x-summary/halfcheetah.pdf}}
    \hspace{-3.5mm}
    \subfigure{
    \includegraphics[scale=0.125]{50+x-2/halfcheetah-medium-v2-50-0.pdf}}
    \hspace{-3.5mm}
    \subfigure{
    \includegraphics[scale=0.125]{50+x-2/halfcheetah-medium-v2-50-5.pdf}}
    \hspace{-3.5mm}
    \subfigure{
    \includegraphics[scale=0.125]{50+x-2/halfcheetah-medium-v2-50-10.pdf}}
    \hspace{-3.5mm}
    \subfigure{
    \includegraphics[scale=0.125]{50+x-2/halfcheetah-medium-v2-50-15.pdf}}
    \hspace{-3.5mm}
    %\subfigure{
    %\includegraphics[scale=0.125]{50+x-2/halfcheetah-medium-v2-50-20.pdf}}
    %\hspace{-3.5mm}
    \subfigure{
    \includegraphics[scale=0.125]{50+x-2/halfcheetah-medium-v2-50-25.pdf}}
    \caption{Experimental results on noised D4RL tasks with various noised trajectories.}
    \label{fig1: performance}
\end{figure*}

\begin{table*}[t]
    \centering
    \begin{tabular}{l|c|c|c|c|c|c|c|c}
         & {\color{blue}BCQ} & {\color{red}BCQ~($\gamma$)} & {\color{blue}CQL} & {\color{red}CQL~($\gamma$)} & {\color{blue}AWAC} & {\color{red}AWAC~($\gamma$)} & {\color{blue}COMBO} & {\color{red}COMBO~($\gamma$)}\\
         \hline
        walker2d (0) & 59.6$\pm$2.7 & 51.5$\pm$3.6 & 65.3$\pm$1.5 & 60.9$\pm$1.4 & 44.8$\pm$2.8 & \textbf{67.5$\pm$1.6} & 26.1$\pm$3.2 & \textbf{65.5$\pm$1.7} \\
        walker2d (10) & 53.7$\pm$2.5 & 51.8$\pm$1.3 & 54.4$\pm$2.7 & \textbf{65.5$\pm$3.2} & 56.6$\pm$1.2 & \textbf{64.8$\pm$4.1} & 47.9$\pm$2.3 & \textbf{63.1$\pm$1.6} \\
        walker2d (50) & 20.3$\pm$3.3 & \textbf{52.4$\pm$3.9} & 62.2$\pm$0.5 & \textbf{68.5$\pm$0.8} & 54.4$\pm$3.2 & \textbf{68.5$\pm$1.9} & 27.2$\pm$1.6 & \textbf{69.6$\pm$1.9} \\
        walker2d (100) & 18.6$\pm$1.9 & \textbf{52.1$\pm$2.2} & 63.1$\pm$1.2 & 57.7$\pm$1.8 & 60.9$\pm$2.6 & \textbf{67.0$\pm$3.2} & 13.3$\pm$1.1 & \textbf{70.7$\pm$2.3} \\
        \hline
        hopper (0) & 52.8$\pm$2.1 & 40.3$\pm$2.5 & 46.3$\pm$0.7 & \textbf{52.5$\pm$1.0} & 49.4$\pm$1.8 & 50.0$\pm$0.7 & 1.5$\pm$0.1 & \textbf{53.5$\pm$3.2}\\
        hopper (10) & 47.9$\pm$2.1 & 41.0$\pm$2.7 & 49.4$\pm$0.4 & \textbf{53.1$\pm$1.6} & 46.3$\pm$0.3 & \textbf{50.4$\pm$0.2} & 1.2$\pm$0.1 & \textbf{56.5$\pm$2.5}\\
        hopper (50) & 12.7$\pm$3.5 & \textbf{44.1$\pm$1.9} & 41.7$\pm$1.1 & \textbf{47.9$\pm$1.3} & 47.9$\pm$1.6 & \textbf{51.9$\pm$1.5} & 1.0$\pm$0.1 & \textbf{48.6$\pm$4.2}\\
        hopper (100) & 1.0$\pm$0.1 & \textbf{41.6$\pm$0.6} & 44.8$\pm$1.9 & \textbf{47.0$\pm$2.5} & 47.3$\pm$0.4 & \textbf{50.0$\pm$2.7} & 1.3$\pm$0.1 & \textbf{52.3$\pm$1.7}\\
        \hline
        halfcheetah (0) & 40.2$\pm$1.3 & \textbf{42.1$\pm$1.1} & 0.8$\pm$0.1 & 0.8$\pm$0.0 & 36.1$\pm$0.6 & \textbf{39.2$\pm$0.3} & 32.6$\pm$1.6 & 27.6$\pm$1.5 \\
        halfcheetah (10) & 39.5$\pm$0.3 & \textbf{40.2$\pm$3.3} & 0.8$\pm$0.0 & 0.9$\pm$0.1 & 35.7$\pm$1.4 & \textbf{38.8$\pm$0.6} & 32.3$\pm$2.8 & 29.7$\pm$2.7 \\
        halfcheetah (50) & 36.5$\pm$0.9 & \textbf{37.8$\pm$0.8} & 0.6$\pm$0.0 & 0.6$\pm$0.0 & 34.6$\pm$1.8 & \textbf{39.6$\pm$0.2} & 31.1$\pm$4.7 & 28.0$\pm$1.6 \\
        halfcheetah (100) & 35.4$\pm$1.1 & \textbf{36.4$\pm$1.7} & 0.7$\pm$0.1 & 0.7$\pm$0.1 & 35.9$\pm$2.0 & \textbf{39.4$\pm$1.8} & 30.0$\pm$1.9 & 29.3$\pm$0.6 \\
        \hline
    \end{tabular}
    \caption{Experimental results on noised D4RL tasks with various offline RL methods.}
    \label{tab1: performance}
\end{table*}

This section investigates whether a reduced discount factor will benefit generalization in a continuous control with a function approximation setting.
Specifically, we evaluate various offline RL algorithms~(TD3+BC, BCQ, CQL, AWAC and COMBO) with a smaller guidance discount factor on the limited D4RL benchmark of OpenAI gym MuJoCo tasks.
The dataset in each task contains 50 medium trajectories and various noised trajectories to approximate the practical scenarios.
The noised trajectories are fragments of the random datasets in D4RL.
To ensure a fair and identical experimental evaluation across algorithms, we re-run these offline algorithms using the author-provided implementation or the recognized code.

We report the final performance results in Table~\ref{tab1: performance} and display the learning curves of TD3+BC in Figure~\ref{fig1: performance}.
The performance of current offline RL methods with original discount facotr~($\gamma=0.99$) degrades with more noisy data due to the less coverage in the dataset.
In contrast, offline RL methods with a small guidance discount factor~($\gamma=0.95$) achieve stable and robust performance in most scenarios.
Besides, we find small data regimes have a noticeable impact on CQL~(e.g., we cannot improve the performance on the halfcheetah task by changing $\gamma$).
Also, training an accurate model with limited data is challenging. 
As a data augmentation version of CQL, the generated state-action pairs of COMBO is noisy~(see the gap between COMBO and COMBO($\gamma$) in walker2d and hopper tasks).
Complete experimental results of TD3+BC on noised D4RL tasks are shown in Appendix~\ref{complete results of TD3+BC}.

\subsubsection{Experimental results of online algorithm}
We evaluate the standard off-policy algorithm TD3 on standard D4RL datasets, which is shown in Figure~\ref{fig2: online algorithm}.
The experimental results show TD3 achieves a noticeable performance improvement on offline tasks with a smaller discount factor, demonstrating the role of the discount factor as a pessimistic mechanism.

\begin{figure}[h]
    \centering
    \subfigure{
    \includegraphics[scale=0.23]{TD3_result/walker2d-medium-v2.pdf}}
    %\hspace{-1.5mm}
    \subfigure{
    \includegraphics[scale=0.23]{TD3_result/halfcheetah-medium-v2.pdf}}
    %\subfigure{
    %\includegraphics[scale=0.23]{TD3_result/walker2d-expert-v2.pdf}}
    \caption{Experimental results of online algorithm TD3 on D4RL datasets.}
    \label{fig2: online algorithm}
\end{figure}

\subsection{Ablation Study}
\subsubsection{Robustness of the small discount factor}
We evaluate TD3+BC on datasets containing 50 medium and 25 noised trajectories with various $\gamma$.
In Figure~\ref{fig3: gamma}, TD3+BC achieves a high performance by decreasing $\gamma$ from 0.99 to around 0.95.
Different offline RL algorithms have minor difference in selecting $\gamma$ on different tasks~(e.g., in Table~\ref{tab1: performance}, BCQ ($\gamma=0.9$) in hopper, CQL ($\gamma=0.98$) in walker2d and COMBO ($\gamma=0.9$) in hopper will be better).
However, the suitable area of $\gamma$ is consistent~($\gamma \in [0.9, 0.95]$), and we don't need to fine-tune $\gamma$ for each task.

\begin{figure}[h]
    \centering
    \subfigure{
    \includegraphics[scale=0.25]{various_gamma/Walker2d-2.pdf}}
    %\hspace{-1.5mm}
    \subfigure{
    \includegraphics[scale=0.25]{various_gamma/Halfcheetah-2.pdf}}
    %\hspace{-1.5mm}
    \subfigure{
    \includegraphics[scale=0.25]{various_gamma/Hopper-2.pdf}}
    \caption{Experimental results on limited D4RL datasets with 25 noised trajectories and TD3+BC algorithm.
    Results are averaged over five simulations and 1000 evaluation episodes.
    Shaded area represents 95\% confidence interval.}
    \label{fig3: gamma}
\end{figure}

\subsubsection{Relationship between $\gamma$ and data size}
We evaluate TD3+BC on datasets containing $x$ medium and 100 noised trajectories.
Then, we select the optimal discount factor $\gamma$ on the performance under different data sizes.
Experimental results in Figure~\ref{fig4: data size} show that the optimal discount factor $\gamma$ increases with the number of trajectories, which is consistent with the theoretical analysis.

\begin{figure}[h]
    \centering
    \subfigure{
    \includegraphics[scale=0.24]{various_datasize/Walker2d.pdf}}
    %\hspace{-1.5mm}
    \subfigure{
    \includegraphics[scale=0.24]{various_datasize/Halfcheetah.pdf}}
    %\hspace{-1.5mm}
    \subfigure{
    \includegraphics[scale=0.24]{various_datasize/Hopper.pdf}}
    \caption{The relationship between optimal $\gamma$ and the number of trajectories.}
    \label{fig4: data size}
\end{figure}

\subsubsection{Comparison between $\gamma$ and $\alpha$ in TD3+BC}
123
